Tensor Generalized Canonical Correlation Analysis

Regularized Generalized Canonical Correlation Analysis (RGCCA) is a general statistical framework for multi-block data analysis. RGCCA enables deciphering relationships between several sets of variables and subsumes many well-known multivariate analysis methods as special cases. However, RGCCA only deals with vector-valued blocks, disregarding their possible higher-order structures. This paper presents Tensor GCCA (TGCCA), a new method for analyzing higher-order tensors with canonical vectors admitting an orthogonal rank-R CP decomposition. Moreover, two algorithms for TGCCA, based on whether a separable covariance structure is imposed or not, are presented along with convergence guarantees. The efficiency and usefulness of TGCCA are evaluated on simulated and real data and compared favorably to state-of-the-art approaches.

==> tables/2B_1000_all.tex <==
\begin{table}
  \caption{Cosine between the true and the estimated canonical vectors as well as computation times.}
    \label{tab:results}
  \centering
  \resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{llll} 
\toprule 
Model & Gas & Cross (little) & Computation time \\ 
\midrule 
2DCCA1 & 0.885 $\pm$ 0.360 & 0.850 $\pm$ 0.270 & 2.916 $\pm$ 0.429 \\ 
TCCA1 & 0.890 $\pm$ 0.009 & 0.855 $\pm$ 0.011 & 7.495 $\pm$ 0.570 \\ 
TGCCA1 & 0.891 $\pm$ 0.009 & 0.858 $\pm$ 0.011 & 19.011 $\pm$ 8.482 \\ 
spTCCA1 & 0.890 $\pm$ 0.272 & 0.852 $\pm$ 0.217 & 7.210 $\pm$ 0.424 \\ 
spTGCCA1 & 0.891 $\pm$ 0.009 & 0.858 $\pm$ 0.014 & 4.817 $\pm$ 0.140 \\ 
CMTF1 & 0.012 $\pm$ 0.020 & 0.208 $\pm$ 0.009 & 12.735 $\pm$ 0.360 \\ 
2DCCA3 & 0.047 $\pm$ 0.085 & 0.026 $\pm$ 0.054 & 1.475 $\pm$ 0.428 \\ 
TCCA3 & 0.890 $\pm$ 0.009 & 0.855 $\pm$ 0.011 & 7.897 $\pm$ 0.453 \\ 
TGCCA3 & 0.871 $\pm$ 0.108 & 0.856 $\pm$ 0.118 & 98.833 $\pm$ 39.858 \\ 
spTCCA3 & 0.890 $\pm$ 0.008 & 0.852 $\pm$ 0.011 & 7.192 $\pm$ 0.194 \\ 
spTGCCA3 & \textbf{0.934 $\pm$ 0.040} & \textbf{0.938 $\pm$ 0.037} & 5.280 $\pm$ 0.587 \\ 
CMTF3 & 0.261 $\pm$ 0.209 & 0.573 $\pm$ 0.228 & 42.519 $\pm$ 9.909 \\ 
RGCCA & 0.197 $\pm$ 0.091 & 0.148 $\pm$ 0.074 & 12.651 $\pm$ 0.450 \\ 
SVD & 0.004 $\pm$ 0.003 & 0.012 $\pm$ 0.008 & 5.180 $\pm$ 0.158 \\ 
\bottomrule 
\end{tabular}
  }%
  
\end{table}

\iffalse
\begin{table}[b]
    \centering
    \resizebox{\columnwidth}{!}{%
\begin{tabular}{||c || c | c | c | c||} 
\hline 
Model & Gas & Cross (little) & Computation time \\ 
\hline\hline 
2DCCA1 & 0.885 $\pm$ 0.360 & 0.850 $\pm$ 0.270 & 2.916 $\pm$ 0.429 \\ 
\hline 
TCCA1 & 0.890 $\pm$ 0.009 & 0.855 $\pm$ 0.011 & 7.495 $\pm$ 0.570 \\ 
\hline 
TGCCA1 & 0.891 $\pm$ 0.009 & 0.858 $\pm$ 0.011 & 19.011 $\pm$ 8.482 \\ 
\hline 
spTCCA1 & 0.890 $\pm$ 0.272 & 0.852 $\pm$ 0.217 & 7.210 $\pm$ 0.424 \\ 
\hline 
spTGCCA1 & 0.891 $\pm$ 0.009 & 0.858 $\pm$ 0.014 & 4.817 $\pm$ 0.140 \\ 
\hline 
2DCCA3 & 0.047 $\pm$ 0.085 & 0.026 $\pm$ 0.054 & 1.475 $\pm$ 0.428 \\ 
\hline 
TCCA3 & 0.890 $\pm$ 0.009 & 0.855 $\pm$ 0.011 & 7.897 $\pm$ 0.453 \\ 
\hline 
TGCCA3 & 0.871 $\pm$ 0.108 & 0.856 $\pm$ 0.118 & 98.833 $\pm$ 39.858 \\ 
\hline 
spTCCA3 & 0.890 $\pm$ 0.008 & 0.852 $\pm$ 0.011 & 7.192 $\pm$ 0.194 \\ 
\hline 
spTGCCA3 & 0.934 $\pm$ 0.040 & 0.938 $\pm$ 0.037 & 5.280 $\pm$ 0.587 \\ 
\hline 
RGCCA & 0.197 $\pm$ 0.091 & 0.148 $\pm$ 0.074 & 12.651 $\pm$ 0.450 \\ 
\hline 
SVD & 0.004 $\pm$ 0.003 & 0.012 $\pm$ 0.008 & 5.180 $\pm$ 0.158 \\ 
\hline 
\end{tabular}

\quad

\begin{tabular}{||c || c | c | c | c||} 
\hline 
Model & Gas & Cross (little) & Computation time \\ 
\hline\hline 
2DCCA1 & 0.908 $\pm$ 0.001 & 0.879 $\pm$ 0.001 & 2.608 $\pm$ 0.508 \\ 
\hline 
TCCA1 & 0.908 $\pm$ 0.001 & 0.879 $\pm$ 0.001 & 7.202 $\pm$ 0.056 \\ 
\hline 
TGCCA1 & 0.908 $\pm$ 0.001 & 0.879 $\pm$ 0.001 & 14.687 $\pm$ 0.380 \\ 
\hline 
spTCCA1 & 0.908 $\pm$ 0.001 & 0.879 $\pm$ 0.001 & 7.057 $\pm$ 0.193 \\ 
\hline 
spTGCCA1 & 0.908 $\pm$ 0.001 & 0.878 $\pm$ 0.001 & 4.718 $\pm$ 0.142 \\ 
\hline 
2DCCA3 & 0.090 $\pm$ 0.049 & 0.093 $\pm$ 0.046 & 1.502 $\pm$ 0.358 \\ 
\hline 
TCCA3 & 0.908 $\pm$ 0.001 & 0.879 $\pm$ 0.001 & 7.556 $\pm$ 0.208 \\ 
\hline 
TGCCA3 & 0.952 $\pm$ 0.010 & 0.842 $\pm$ 0.048 & 159.346 $\pm$ 135.210 \\ 
\hline 
spTCCA3 & 0.908 $\pm$ 0.001 & 0.879 $\pm$ 0.001 & 7.016 $\pm$ 0.262 \\ 
\hline 
spTGCCA3 & 0.982 $\pm$ 0.002 & 0.990 $\pm$ 0.001 & 5.102 $\pm$ 0.236 \\ 
\hline 
RGCCA & 0.977 $\pm$ 0.003 & 0.986 $\pm$ 0.002 & 10.544 $\pm$ 0.120 \\ 
\hline 
SVD & 0.989 $\pm$ 0.008 & 0.991 $\pm$ 0.011 & 5.144 $\pm$ 0.151 \\ 
\hline 
\end{tabular}
    }%
    \caption{Cosine between the true canonical vectors and the estimated ones for different models on block "Gas" and "Cross (little)" for levels of SNR 0.1 (left table) and 1 (right table) as well as the computation time.}
    \label{tab:results}
\end{table}
\fi

==> tables/5B_1000_all.tex <==
\begin{table}
  \caption{Cosine between the true canonical vectors and the estimated ones as well as computation times for level of SNR -20dB.}
    \label{tab:results5B}
  \centering
  \resizebox{\columnwidth}{!}{%
  \input{appendix/tables/raw_tables/5B_1000_all/table_SNR_0.1.txt}
  }
\end{table}

==> tables/5blocks.tex <==
\begin{table}[b]
\caption{Description of the generated blocks.}
    \label{tab:blocks}
    \centering
    \resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{llllll} 
\toprule 
Block & Name & Structure & Folded shape & Rank & Used in $L = 2$ setting? \\ 
\midrule
1 & Square & matrix & 30 $\times$ 35 & 1 & $\times$ \\
2 & Gas & matrix & 45 $\times$ 38 & 12 & $\checkmark$ \\
3 & Cross & matrix & 38 $\times$ 38 & 2 & $\times$ \\
4 & Cross (little) & matrix & 19 $\times$ 19 & 2 & $\checkmark$ \\
5 & Vector & vector & 100 & NA & $\times$ \\
\bottomrule
\end{tabular}
    }%
\end{table}

==> tables/blocks.tex <==
\begin{table}
  \caption{Description of the generated blocks in the $L = 2$ setting.}
  \label{tab:blocks}
  \centering
  \resizebox{0.8\columnwidth}{!}{%
  \begin{tabular}{llll}
    \toprule
    Block & Name & Folded shape & Rank \\ 
    \midrule
    1 & Gas & 45 $\times$ 38 & 12 \\
    2 & Cross (little) & 19 $\times$ 19 & 2 \\
    \bottomrule
  \end{tabular}
  }%
\end{table}


